Catchphrase: Automatic Detection of Cultural References

A snowclone is a customizable phrasal template that can be realized in multiple, instantly recognized variants. For example, ``* is the new *" (Orange is the new black, 40 is the new 30). Snowclones are extensively used in social media. In this paper, we study snowclones originating from pop-culture quotes; our goal is to automatically detect cultural references in text. We introduce a new, publicly available data set of pop-culture quotes and their corresponding snowclone usages and train models on them. We publish code for Catchphrase, an internet browser plugin to automatically detect and mark references in real-time, and examine its performance via a user study. Aside from assisting people to better comprehend cultural references, we hope that detecting snowclones can complement work on paraphrasing and help to tackle long-standing questions in social science about the dynamics of information propagation.

==> tasks_and_data.tex <==
\remove{
\section{Tasks and Data}
\nnote{I used the first subsection to formally describe the tasks, and the second to describe the data sets we've created. I think the definitions of the models we're looking for M,T can be better edited}
\label{sec:task and data}
%Motivated by the results of the user-study discussed in \ref{snowclone tagging task}, we formally define the 2 main tasks we set to solve. 






\subsection{Data Sets} In order to study both tasks, we create 2 new publicly
\label{datasets}
available data sets. As to our knowledge, there are no other data sets available for these tasks. 
\paragraph{Snowclone-form data set}For the first task, 

}
